Consistent Estimation for PCA and Sparse Regression with Oblivious Outliers

We develop machinery to design efficiently computable and consistent estimators, achieving estimation error approaching zero as the number of observations grows, when facing an oblivious adversary that may corrupt responses in all but an $\alpha$ fraction of the samples. As concrete examples, we investigate two problems: sparse regression and principal component analysis (PCA). For sparse regression, we achieve consistency for optimal sample size $n\gtrsim (k\log d)/\alpha^2$ and optimal error rate $O(\sqrt{(k\log d)/(n\cdot \alpha^2)})$ where $n$ is the number of observations, $d$ is the number of dimensions and $k$ is the sparsity of the parameter vector, allowing the fraction of inliers to be inverse-polynomial in the number of samples. Prior to this work, no estimator was known to be consistent when the fraction of inliers $\alpha$ is $o(1/\log \log n)$, even for (non-spherical) Gaussian design matrices. Results holding under weak design assumptions and in the presence of such general noise have only been shown in dense setting (i.e., general linear regression) very recently by d'Orsi et al. [dNS21]. In the context of PCA, we attain optimal error guarantees under broad spikiness assumptions on the parameter matrix (usually used in matrix completion). Previous works could obtain non-trivial guarantees only under the assumptions that the measurement noise corresponding to the inliers is polynomially small in $n$ (e.g., Gaussian with variance $1/n^2$). To devise our estimators, we equip the Huber loss with non-smooth regularizers such as the $\ell_1$ norm or the nuclear norm, and extend d'Orsi et al.'s approach [dNS21] in a novel way to analyze the loss function. Our machinery appears to be easily applicable to a wide range of estimation problems.

==> content/check-list.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%	justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%	\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%	\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%	\item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
		\answerYes
		\item Did you describe the limitations of your work?
		\answerYes See Section~\ref{sec:results}.
		\item Did you discuss any potential negative societal impacts of your work?
		\answerNA This work does not present any foreseeable societal consequence.
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes
	\end{enumerate}
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerYes See Section~\ref{sec:results}.
		\item Did you include complete proofs of all theoretical results?
		\answerYes See Supplementary Material	.
	\end{enumerate}
	
	\item If you ran experiments...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerNA{}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerNA{}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerNA{}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerNA{}
	\end{enumerate}
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerNA{}
		\item Did you mention the license of the assets?
		\answerNA{}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerNA{}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerNA{}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerNA{}
	\end{enumerate}
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
		\answerNA{}
	\end{enumerate}
	
\end{enumerate}


==> content/literature-pca.tex <==

\Cnote{The following is some history for robust PCA. It is not necessary to include all of them. We may just use some phrases to introduce.}

\emph{Principal Component Analysis} (PCA) is one of the most widely used statistical tools for high-dimensional data analysis in the scenario that the data approximately lie on a low-dimensional subspace.
Mathematically, all data points are formulated as the column vectors of a matrix $M$ such that
$M=L_0+Z_0$ where $L_0$ is a low-rank matrix and $Z_0$ is a small perturbation matrix.
Then, PCA seeks the best rank-$k$ estimate of $L_0$ in the $\ell_2$ sense, i.e., $\argmin_{\mathrm{rank}(L)\leq k} \normt{M-L}$.
This optimization problem can be solved efficiently via singular value decomposition and thresholding.

However, the classical PCA breaks down even with a single grossly corrupted entry, limiting its applicability in diverse area. 
To recover a low-rank matrix $L_0$ from a highly corrupted data matrix $M$, instead of $N_0$, a formulation of \emph{robust PCA} adopts a sparse matrix $S_0$ whose entries have arbitrary large magnitude such that $M=L_0+S_0$.
Remarkably, Cand\`{e}s et al.~\cite{DBLP:journals/jacm/CandesLMW11} showed that under certain conditions, the convex relaxation, $\argmin_{L+S=M}\normn{L}+\frac{1}{\sqrt{n}}\normo{S}$, can exactly recover $L_0$ and $S_0$ with high probability.

Furthermore, since the observations in real world applications are often corrupted by noise, Zhou et al.~\cite{DBLP:conf/isit/ZhouLWCM10} included the noise matrix $Z_0$ again and formulated \emph{stable PCA} as $M=L_0+S_0+Z_0$ with $\normf{Z_0}\leq \rho$. 
Based on Cand\`{e}s et al. results, they further proved that the convex relaxation,  $\argmin_{\normf{M-L-S}\leq \rho}\normn{L}+\frac{1}{\sqrt{n}}\normo{S}$, yields an approximate solution $(\hat{L},\hat{S})$ such that with high probability,  $\normf{\hat{L}-L_0}^2+\normf{\hat{S}-S_0}=O(\rho^2n^2)$. 

Nevertheless, Cand\`{e}s et al.'s  and Zhou et al.'s proofs highly depend on the \emph{incoherence} of the low-rank matrix $L_0$. 
Roughly speaking, the singular vectors of $L_0$ should not be ``aligned'' with standard coordinate vectors. 
Therefore, this incoherence condition significantly restricts practical applications using their results.
